Joint Wasserstein Distribution Matching

Joint distribution matching (JDM) problem, which aims to learn bidirectional mappings to match joint distributions of two domains, occurs in many machine learning and computer vision applications. This problem, however, is very difficult due to two critical challenges: (i) it is often difficult to exploit sufficient information from the joint distribution to conduct the matching; (ii) this problem is hard to formulate and optimize. In this paper, relying on optimal transport theory, we propose to address JDM problem by minimizing the Wasserstein distance of the joint distributions in two domains. However, the resultant optimization problem is still intractable. We then propose an important theorem to reduce the intractable problem into a simple optimization problem, and develop a novel method (called Joint Wasserstein Distribution Matching (JWDM)) to solve it. In the experiments, we apply our method to unsupervised image translation and cross-domain video synthesis. Both qualitative and quantitative comparisons demonstrate the superior performance of our method over several state-of-the-arts.

==> supp_backups.tex <==
\onecolumn
\vskip 0.3in
\clearpage
\textbf{\Large{~~~~~Supplementary Materials for ``Joint Wasserstein Distribution Matching''}}
\vspace{20pt}
%\begin{Large}
% 	~~~~~~~~~~Supplementary Materials for ``Joint Wasserstein Distribution Matching''
%% 	~~~~~~~~~~~~{\large{Supplementary Materials}}: ``J{\large{OINT}} W{\large{ASSERSTEIN}} D{\large{ISTRIBUTION}}-E{\large{ATCHING}}''
%\end{Large}
%\title{Joint Wasserstein Distribution Matching}
%\begin{appendix}

\setcounter{section}{0}

\section{Theoretical Analysis}\label{sec:theory}  %Wasserstein Distance of Joint Distributions
%{To learn a joint distribution, one can learn a shared latent space for two different domains~\citep{liu2017unsupervised}.}
%%Based on the shared-latent space assumption~\citep{liu2017unsupervised}, 
%In this sense, any pair of images in different domains can be mapped to the same latent representation. % in a shared-latent space.
%We define latent variable models $ P_{G_1} $ and $ P_{G_2} $ by a two-step procedure: first a code $ Z {\in} \gZ $ is sampled from some prior distribution $ P_{Z} $ and then $ Z $ can be mapped to $ X $ and $ Y $, respectively. 
%Then, we have the following densities:% of the form:
%\begin{align}\label{eq:G1G2}
%	p_{G_1}(\rvx) {:=} \int_{\gZ} p_{G_1}(\rvx|\rvz) p_{\rvz}(\rvz) d\rvz, \forall\; \rvx {\in} \gX, \quad\;
%	p_{G_2}(\rvy) {:=} \int_{\gZ} p_{G_2}(\rvy|\rvz) p_{\rvz}(\rvz) d\rvz, \forall\; \rvy {\in} \gY,
%\end{align}
%where all involved densities are properly defined.
%In this paper, we focus on non-random decoders $ G_1{:\;} \gZ {\to} \gX $ and $ G_2{:\;} \gZ {\to} \gY $, \textit{i.e.}, generative models $ P_{G_1}(X'|Z) $ and $ P_{G_2}(Y'|Z) $ deterministically mapping $ Z $ to $ X' {=} G_1(Z) $ and $ Y' {=} G_2(Z) $, respectively.
%Based on these two models, we then construct joint distributions in two domains and define the following Wasserstein distance.
%
To address the joint distribution matching problem, one can learn a shared latent space $ \gZ $ in two domains~\cite{liu2017unsupervised}.
In this sense, any pair of images in different domains can be mapped to the same latent representation. 
Inversely, there exist generative models $ P_{G_1}(X'|Z) $ and $ P_{G_2}(Y'|Z) $ that map a shared latent code $ Z $ to $ X' {=} G_1(Z) $ and $ Y' {=} G_2(Z) $, respectively.
%\textbf{Wasserstein distance between joint distributions.}
Then $ P_{\gA} (X, Y') $ and $ P_{\gB} (X', Y) $ are two joint distributions between real and generated images, 
%, where $ X' $ and $ Y' $ are sampled from the models $ {G_1} $ and $ {G_2} $, respectively, and $ X $ and $ Y $ are true images from different domains.
%For the unsupervised joint distribution matching problem,
%Based on the optimal transport theory~\cite{villani2008optimal}, 
we define Wasserstein distance $ \gW_c(P_{\gA},  P_{\gB}) $ as %between joint distributions $ P_{\gA} $ and $ P_{\gB} $, \textit{i.e.},
%Our goal is to find a optimal coupling to make these two joint distributions to close to each other.
\begin{align} \label{pro:joint_ot}
\gW_c(P_{\gA},  P_{\gB}) \mathop{=} \min_{P {\in} \gP(P_{\gA}, P_{\gB})}
\E_{P} [c(X, Y'; X', Y)],
\end{align}
where $ \gP(P_{\gA}, P_{\gB}) $ is the set of couplings composed of joint  distributions with the probability distributions $ (P_{\gA},  P_{\gB}) $. %, and $ c $ is a  cost function. 
In practice, we set the cost function $ c(X, Y'; X', Y) = c_1(X, X') + c_2(Y', Y) $ \cite{damodaran2018deepjdot}, where $ c_1 $ and $ c_2 $ can be any metric.
% between two joint probability distributions $ P_{\gA} $ and $ P_{\gB} $.
%When $ (\gX {\times} \gY)^2 $ is equipped with a metric $ d $, a typical choice is to set $ c (\rvx, \rvy'; \rvx', \rvy) {=} d(\rvx, \rvy'; \rvx', \rvy)^p $, where $ p > 0 $. For $ p \ge 1 $, $ \gW^p(P_{\gA},  P_{\gB}) $ is the $ p $-Wasserstein distance between the probability distributions $ (P_{\gA},  P_{\gB}) $.
%there are an important challenges on Wasserstein distance and the cost function.
\kui{However, directly optimizing Problem (\ref{pro:joint_ot})  would incur intractable computation cost and statistical difficulties~\cite{genevay2018learning}.  To address this, we first reduce the intractable Problem (\ref{pro:joint_ot}) into a simpler optimization problem using the following Theorem \ref{thm:opt}.}  \\
%To address this, we need to propose a new optimization method for our problem setting.
%in the unsupervised image-to-image translation task.
%Second, how to choose a appropriate cost function is very challenging.
%In this paper, we set $ c(X, Y'; X', Y) = c_1(X, X') + c_2(Y', Y) $~\citep{damodaran2018deepjdot}, where $ c_1 $ and $ c_2 $ can be any metric to measure the distance in $ \gX {\times} \gX $ and $ \gY {\times} \gY $, respectively. 
%This cost function 
%Here, we set $ \lambda{=}1 $ for convenience.
%, and $ \lambda $ is a positive parameter which balances $ c_1 $ and $ c_2 $ in the their corresponding feature spaces.
%\cao{Then, we derive the following theorem so that the intractable Problem (\ref{pro:joint_ot}) can be reduced to a simple optimization problem.}
%\kui{Give more clear definitions about $Q$ here!!!} 
\emph{
\noindent\textbf{\emph{Theorem \ref{thm:equ_problem}}} (\textbf{Problem equivalence})
	Assume that two domains share the same latent space, then Wasserstein distribution between joint distributions can be defined as
	\begin{equation}
	\begin{aligned}  \label{prob:equ_problem}
	\gW_c(\gP_{\gA}, \gP_{\gB}) &= \gR_x(F) + \gR_y(F), \\
	\st \quad P_X &= Q_X, P_Y = Q_Y, P_Z = Q_Z,
	\end{aligned}
	\end{equation}
	where $ \gR_x (F)$ and $\gR_y(F) $ are reconstruction losses \wrt Auto-Encoders $ G_1{\circ} E_1 $ and $ G_2 {\circ} E_2 $. For convenience, we let $ F{=}\{E_1, E_2, G_1, G_2\} $. Here, $ P_X, P_Y $ and $ P_Z $ are real distributions, and $ Q_X, Q_Y $ and $ Q_Z $ are generated distributions.
}

\begin{proof}
From Theorem \ref{thm:opt}, we define the reconstruction losses as:
\begin{align*}
	\gR_x(F) = \E_{P_{X}} \E_{Q{(Z_1|X)}}  [c_1(X, G_1(Z_1))]\quad \text{and} \quad \gR_y(F) = \E_{P_{Y}} \E_{Q{(Z_2|Y)}} [c_2(G_2(Z_2), Y)],
\end{align*}
where $ c_1(X, G_1(Z_1))=\| X- G_1(Z_1) \|_1 $ and $ c_2(G_2(Z_2), Y)=\| G_2(Z_2)- Y \|_1 $ in this paper. 
For the constraints in this problem, we enforce the constraints in Theorem \ref{thm:opt}, $ P_X {=} Q_X, P_Y {=} Q_Y $ and $ P_{Z_1}{=}Q_{Z_1}, P_{Z_2}{=}Q_{Z_2} $. 
Note that $ P_{Z_1} {=} P_{Z_2} $, and they are prior distributions. 
We let $ P_Z{:=} \{P_{Z_1}, P_{Z_2}\} $ and $ Q_Z{:=} \{Q_{Z_1}, Q_{Z_2} \} $, then we have $ P_Z = Q_Z $.

\end{proof}
%\vspace{15pt}


\kui{Let $ Q(Z_1|X) $ and $ Q(Z_2|Y) $ be two probabilistic encoders,} where $ X {\sim} P_{X}  $ and $ Y {\sim} P_{Y} $,
and $ Q_{Z_1} $ and $ Q_{Z_2} $ be two marginal distributions: \cao{$Q_{Z_1} {=} \E_{P_X}[Q(Z_1|X)]$ and $Q_{Z_2} {=} \E_{P_Y}[Q(Z_2|Y)]$}.  %of $ Z_1 {\sim} Q(Z_1|X) $ and $ Z_2 {\sim} Q(Z_2|Y) $, respectively
% We define the sets of all probabilistic encoders as $ \gQ_1 {=} \{Q(Z_1|X) |\; Q {\in} \tilde{\gQ}, P_Y {=} Q_{Y} \} $, $ \gQ_2 {=} \{Q(Z_2|Y) |\; Q {\in} \tilde{\gQ}, P_X {=} Q_{X} \} $ \cao{where $Q$ satisfies the set $\tilde{\gQ} {=} \{ Q| P_{Z_1} {=} Q_{Z_1}, P_{Z_2} {=} Q_{Z_2} \} $}. %
Then, we can achieve an equivalent problem to Problem (\ref{pro:joint_ot}) as follows.

\begin{thm}\label{thm:opt}
	Given two deterministic models $ P_{G_1} (X'|Z) $ and $ P_{G_2} (Y'|Z) $ as Dirac measures, \textit{i.e.},
	$ P_{G_1}({X'}|Z{=}\rvz){=}\delta_{G_1(\rvz)} $ and $ P_{G_2}(Y'|Z{=}\rvz){=}\delta_{G_2(\rvz)} $ for all $ \rvz {\in} \gZ $, we can rewrite Problem (\ref{pro:joint_ot}) as follows:
	%\begin{equation}
	%\begin{aligned}\label{obj:w}
	\begin{align} \label{obj:w}
	\gW_c(P_{\gA}, P_{\gB})
	{=}& \inf_{Q  {\in} \gQ_1} \E_{P_{X}} \E_{Q{(Z_1|X)}}  [c_1(X, G_1(Z_1))] \\
	&\tiny{+}\inf_{Q {\in} \gQ_2} \E_{P_{Y}} \E_{Q{(Z_2|Y)}} [c_2(G_2(Z_2), Y)], \nonumber
	\end{align}
	where we define $ \gQ_1 {=} \{Q(Z_1|X) |\; Q {\in} \tilde{\gQ}, P_Y {=} Q_{Y} \} $ and $ \gQ_2 {=} \{Q(Z_2|Y) |\; Q {\in} \tilde{\gQ}, P_X {=} Q_{X} \} $ as the sets of all probabilistic encoders, respectively,  \cao{where $Q$ satisfies the set $\tilde{\gQ} {=} \{ Q| P_{Z_1} {=} Q_{Z_1}, P_{Z_2} {=} Q_{Z_2} \} $}.
	%\end{aligned}
	%\end{equation}
	%\footnote{See supplementary materials for the proof.}
\end{thm}


% \begin{remark}
%     Theorem \ref{thm:opt} indicates that Problem \ref{obj:w} is equivalent to Problem \ref{pro:joint_ot}. 
%     %$  G_2{\circ}E_1  $ and $  G_1 {\circ}E_2 $ to generate samples $ Y' $ and $ X' $ such that the generated distribution is close to real distribution.
%     Moreover, latent distributions learned by two probabilistic encoders (\ie ) should be close to each other.
% \end{remark}

%As previously mentioned, finding an optimal couplings between $ P_{\gA} $ and $ P_{\gB} $ is very challenging. Fortunately, according to Theorem \ref{thm:opt}, we can instead optimize problem (\ref{obj:w}) for joint distribution matching. 
%The objective function and detailed optimizations are given below.
%Theorem \ref{thm:opt} allows us to construct an optimization problem by optimizing $ Q(Z_1|X) $ and $ Q(Z_2|Y) $ instead of finding an optimal couplings between joint distributions $ P_{\gA} $ and $ P_{\gB} $.

\begin{proof}
	We denote by $ \gP(X {\sim} P_X, {X'} {\sim} P_{G_1}) $ and $ \gP(Y {\sim} P_Y, {Y'} {\sim} P_{G_2}) $ the set of all joint distributions of $ (X, {X'}) $ and $ (Y, {Y'}) $ with marginals $ P_X, P_{G_1} $ and $ P_Y, P_{G_2} $, respectively,
	and denote by $ \gP(P_{\gA}, P_{\gB}) $ the set of all joint distribution of $ P_{\gA} $ and $ P_{\gB} $. Recall the definition of Wasserstein distance $ \gW_c(P_{\gA}, P_{\gB}) $, we have
	\begin{align}
	\gW_c(P_{\gA}, P_{\gB}) 
	=& \inf_{\pi \in \gP(P_{\gA}, P_{\gB})} \E_{(X, Y'; X', Y) \sim \pi} [ c(X, Y'; X', Y)] \label{eqn:AE1}\\
	=& \inf_{\pi \in \gP(P_{\gA}, P_{\gB})} \E_{(X, Y'; X', Y) \sim \pi} [ c_1(X, X') ] 
	+ \inf_{\pi \in \gP(P_{\gA}, P_{\gB})} \E_{(X, Y'; X', Y) \sim \pi} [ c_2(Y', Y) ] \nonumber \\
	=& \inf_{P \in \gP_{X, X'}} \E_{(X, X') \sim P} [c_1(X, X')] 
	+ \inf_{P \in \gP_{Y, Y'}} \E_{(Y', Y) \sim P} [ c_2(Y', Y)] \label{eqn:AE2}\\
	=& \inf_{P \in \gP({P_{X}, P_{G_1}})} \E_{(X, X') \sim P} [c_1(X, X')] 
	+ \inf_{P \in \gP({P_{Y}, P_{G_2}})} \E_{(Y', Y) \sim P} [ c_2(Y', Y)] \label{eqn:AE3}\\
	=& \;\gW_{c_1}(P_{X}, P_{G_1}) +  \gW_{c_2}(P_{G_2}, P_{Y}). \nonumber
	\end{align}
	Line (\ref{eqn:AE1}) holds by the definition of $ \gW_c(P_{\gA}, P_{\gB})  $.
%	The second line holds by the choose of the ground cost, \textit{i.e.}, $ c(X, Y'; X', Y ) {=}  c_1(X, X') +  c_2(Y', Y) $. 
	Line (\ref{eqn:AE2}) uses the fact that the variable pair $ (X, X') $ is independent of the variable pair $ (Y, Y') $, and $ \gP_{X, X'} $ and $ \gP_{Y, Y'} $ are the marginals on $ (X, X') $ and $ Y, Y' $ induced by joint distributions in $ \gP_{X, Y', X', Y} $. 
	In Line (\ref{eqn:AE3}), if $ P_{G_1}(X'|Z) $ and $ P_{G_2}(Y'|Z) $ are Dirac measures (\textit{i.e.}, $ X' {=} G_1(Z) $ and $ Y' {=} G_2(Z) $), we have 
	\[\gP_{X, X'} {=} \gP(P_X, P_{G_1}), \qquad \gP_{Y, Y'} {=} \gP(P_Y, P_{G_2}). \]
	We consider certain sets of joint probability distributions $ \gP_{X, X', Z_1} $ and $ \gP_{Y, Y', Z_2} $ of three random variables $ (X, X', Z_1) \in \gX {\times} \gX {\times} \gZ $ and $ (Y', Y, Z_2) \in \gY {\times} \gY {\times} \gZ $, respectively. 
	%	We denote by $ P_{G_1, Z}(X', Z) $ and $ P_{G_2, Z}(Y', Z) $ joint distributions of variable pairs $ (X', Z) $ and $ (Y', Z) $, respectively, where $ Z $ is first sampled from $ P_Z $ and then $ X' $ from $ P_{G_1}(X'|Z) $ and $ Y' $ from $ P_{G_2}(Y'|Z) $, respectively.
	%	Note that $ P_{G_1} $ and $ P_{G_2} $ defined in (\ref{eq:G1G2}) are the marginal distributions of $ X' $ and $ Y' $ when $ (X', Z) {\sim} P_{G_1, Z} $ and $ (Y', Z) {\sim} P_{G_2, Z} $.
	We denote by $ \gP(X {\sim} P_X, Z_1 {\sim} P_{Z_1}) $ and $ \gP(Y {\sim} P_Y, Z_2 {\sim} P_{Z_2}) $ the set of all joint distributions of $ (X, Z_1) $ and $ (Y, Z_2) $ with marginals $ P_X, P_{Z_1} $ and $ P_Y, P_{Z_2} $, respectively.
	The set of all joint distributions $ \gP_{X, X', Z_1} $ such that $ X {\sim} P_X, (X', Z_1) {\sim} P_{G_1, Z_1} $ and $ (X' {\Perp} X) | Z_1 $, and likewise for $ \gP_{Y, Y', Z_2} $.
	We denote by $ \gP_{X, X'} $ and $ \gP_{X, Z_1} $ the sets of marginals on $ (X, X') $ and $ (X, Z_1) $ induced by distributions in $ \gP_{X, X', Z_1} $, respectively, and likewise for $ \gP_{Y, Y'} $ and $ \gP_{Y, Z_2} $.
	%	Since the latent variable $ Z $ is related to $ P_{G_1} $ and $ P_{G_2} $, we 
	For the further analyses, we have
%	\begin{small}
	\begin{align}
	&\gW_{c_1}(P_{X}, P_{G_1}) +  \gW_{c_2}(P_{Y}, P_{G_2}) \nonumber\\
	{=}& \inf_{P \in \gP_{X, X', Z_1}} \E_{(X, X', Z_1) \sim P} [ c_1(X, X') ] \label{eqn:ae1}
	 {+} \inf_{P \in \gP_{Y', Y, Z_2}} \E_{(Y', Y, Z_2) \sim P} [  c_2(Y', Y) ]  \\
	{=}& \inf_{P \in \gP_{X, X', Z_1}} \E_{P_{Z_1}} \E_{X \sim P(X|Z_1)} \E_{X' \sim P(X'|Z_1)} [ c_1(X, X') ] \label{eqn:ae2} \\
	 &{+} \inf_{P \in \gP_{Y', Y, Z_2}} \E_{P_{Z_2}} \E_{Y \sim P(Y|Z_2)} \E_{Y' \sim P(Y'|Z_2)} [ c_2(Y', Y) ] \nonumber \\
	{=}& \inf_{P \in \gP_{X, X', Z_1}} \E_{P_{Z_1}} \E_{X \sim P(X|Z_1)} [ c_1(X, G_1(Z_1)) ] 
	 {+} \inf_{P \in \gP_{Y', Y, Z_2}} \E_{P_{Z_2}} \E_{Y \sim P(Y|Z_2)} [ c_2(G_2(Z_2), Y) ] \nonumber \\
	{=}& \inf_{P \in \gP_{X, Z_1}} \E_{(X, Z_1) \sim P} [ c_1(X, G_1(Z_1)) ]  
	 {+} \inf_{P \in \gP_{Y, Z_2}} \E_{(Y, Z_2) \sim P} [ c_2(G_2(Z_2), Y) ] \label{eqn:ae4} \\
	{=}& \inf_{P \in \gP(X, Z_1)} \E_{(X, Z_1) {\sim} P} [ c_1(X, G_1(Z_1)) ] 
	 {+} \inf_{P \in \gP(Y, Z_2)} \E_{(Y, Z_2) {\sim} P} [ c_2(G_2(Z_2), Y) ] \label{eqn:ae5} \\
	{=}& \inf_{Q \in \gQ_1} \E_{P_{X}} \E_{Q{(Z_1|X)}} [c_1(X, G_1(Z_1))] 
	 {+} \inf_{Q \in \gQ_2} \E_{P_{Y}} \E_{Q{(Z_2|Y)}} [c_2(G_2(Z_2), Y)], \label{eqn:ae6} 
	\end{align}
%	\end{small}
	where $ \gQ_1 {=} \{Q(Z_1|X) | Q_{Z_1} {=} P_Z {=} Q_{Z_2}, P_Y {=}  Q_{Y} \} $ and $ \gQ_2 {=} \{Q(Z_2|Y) | Q_{Z_1} {=} P_Z {=} Q_{Z_2}, P_X {=} Q_{X}\} $ are the set of all probabilistic encoders, where $ Q_{Z_1} $ and $ Q_{Z_2} $ are the marginal distributions of $ Z_1 {\sim} Q(Z_1|X) $ and $ Z_2 {\sim} Q(Z_2|Y) $, where $ X {\sim} P_{X}  $ and $ Y {\sim} P_{Y} $, respectively.  
	 
	Line (\ref{eqn:ae1}) uses the tower rule of expectation and Line (\ref{eqn:ae2}) holds by the conditional independence property of $ \gP_{X, X', Z} $. 
%	In line (\ref{eqn:ae3}), we take the expectation w.r.t. the models $ P(X|Z_1) $ and $ P(Y|Z_2) $, respectively.
	In line (\ref{eqn:ae4}), we take the expectation w.r.t. $ X' $ and $ Y' $, respectively, and use the total probability.
	Line (\ref{eqn:ae5}) follows the fact that $ \gP_{X, Z_1} {=} \gP(X {\sim} P_X, Z_1 {\sim} P_{Z_1}) $ and $ \gP_{Y, Z_2} {=} \gP(Y {\sim} P_Y, Z_2 {\sim} P_{Z_2}) $ since $ \gP(P_X, P_{G_1}), \gP_{X, X', Z_1} $ and $ \gP_{X, Y} $ depend on the choice of conditional distributions $ P_{G_1}(X'|Z_1) $, while $ P_{X, Z_1} $ does not, and likewise for distributions w.r.t. $ Y $ and $ G_2 $. 
	In line (\ref{eqn:ae6}), the generative model $ Q(Z_1|X) $ can be derived from two cases where $ Z_1 $ can be sampled from $ E_1(X) $ and $ E_2(G_2(E_1(X))) $ when $ Q_{Z_1} {=} Q_{Z_2} $ and $ P_Y {=} Q_{Y} $, and likewise for the generative model $ Q(Z_2|Y) $.
\end{proof}
%
%\section{Proof of Theorem \ref{theorem}}
%
%\begin{lemma}\label{lemma:dual_KR}
%	Given an $ L_{c_2} $-Lipschitz cost function $ c_2 $, a probabilistic cross-domain Lipschitz function $ f^* $, and two joint distributions $ P_{\gA}^f $ and $ P_{\gB}^g $ w.r.t. $ f $ and $ g $, respectively, then for any coupling $ P( X, Y^f; X^g, Y) \in \gP(P_{\gA}^f, P_{\gB}^g) $, we have
%	\begin{align*}
%		\left| \int_{\gX \times \gY} c_2 (Y, f^*(X)) d ( P_{\gA}^f {-} P_{\gB}^g ) \right| 
%		{\leq} \int_{(\gX \times \gY)^2} \left| c_2 (Y^f, f^*(X)) {-} c_2(Y, f^*(X^g)) \right|d P( X, Y^f; X^g, Y),
%	\end{align*}
%	where $ P_{\gA}^f {=} (X, Y^f)_{X \sim P_X} $ and $ P_{\gB}^g {=} (X^g, Y)_{Y {\sim} P_Y}  $, and $ Y^f {=} f(X) $ and $ X^g {=} g(Y) $.
%\end{lemma}
%\begin{proof}
%	Given joint distributions $ P_{\gA}^f {=} (X, f(X))_{X \sim P_X} $ and $ P_{\gB}^g {=} (g(Y), Y)_{Y {\sim} P_Y} $, and an $ L_{c_2} $-Lipschitz cost function $ c_2 $ on $ \gY \times \gY $, 
%	and based on the duality form of the Kantorovitch-Rubinstein theorem \cite{rachev1990duality, villani2008optimal}, we have
%	\begin{align*}
%	\sup \int_{\gX \times \gY} c_2 (Y, f^*(X)) d ( P_{\gA}^f - P_{\gB}^g ) 
%	= \inf \int_{(\gX \times \gY)^2} d_{f^*}(X, Y^f; X^g, Y) d P (X, Y^f; X^g, Y)
%	\end{align*}
%	where $ d_{f^*}(X, Y^f; X^g, Y) $ is a cost function of $ f^* $ w.r.t. $ (X, Y^f; X^g, Y) $, and the cost function $ c_2 $ satisfies the condition, \textit{i.e.}, $ c_2 (Y^f, f^*(X)) - c_2 (Y, f^*(X^g)) \leq d_{f^*} (X, Y^f; X^g, Y) $. Specifically, we choose its equality , then we have
%	\begin{align*}
%		& \left|\int_{\gX \times \gY} c_2 (Y, f^*(X)) d ( P_{\gA}^f - P_{\gB}^g ) \right|\\
%		\leq& \left| \int_{(\gX \times \gY)^2} c_2 (Y^f, f^*(X)) - c_2 (Y, f^*(X^g)) d P (X, Y^f; X^g, Y) \right|\\
%		\leq& \int_{(\gX \times \gY)^2} \left|  c_2 (Y^f, f^*(X)) - c_2 (Y, f^*(X^g)) \right| d P (X, Y^f; X^g, Y).
%	\end{align*}
%\end{proof}
%
%\begin{lemma}
%	Given an $ L_{c_1} $-Lipschitz cost function $ c_1 $, two joint distributions $ P_{\gA}^f $ and $ P_{\gB}^g $, and a $ \phi(\alpha) $-probabilistic cross-domain Lipschitz function $ f^* $, we assume the input space $ \gX $ is bounded such that $ \| f^*(X_1) - f^*(X_2) \| \leq M_1 $, then we have
%	\begin{align*}
%	\left| E_{\gA}^f (f^*) - E_{\gB}^g (f^*) \right| \leq \gW (P_{\gA}^f, P_{\gB}^g) + L_{c_1} M_1 \phi(\alpha).
%	\end{align*}
%\end{lemma}
%\begin{proof}
%	Based on the definition of $ E_{\gA}^f (f^*) $ and $ E_{\gB}^g (f^*) $, we discuss the absolute value of the difference between them as follows:
%	\begin{small}
%	\begin{align}
%	&\left| E_{\gA}^f (f^*) - E_{\gB}^g (f^*) \right| \nonumber \\
%	=& \left| \E_{(X, Y) \sim P_{\gA}^f(X, Y)} \left[ c_2 (Y, f^*(X)) \right] - \E_{(X, Y) \sim P_{\gB}^g(X, Y)} \left[ c_2 (Y, f^*(X)) \right] \right| \nonumber\\ 
%%	=& \left| \int_{\gX \times \gY} c_2 (Y, f^*(X)) \left( p_{\gA}^f(X, Y) - p_{\gB}^g(X, Y) \right) d X d Y \right| \\
%	=& \left| \int_{\gX \times \gY} c_2 (Y, f^*(X)) d \left( P_{\gA}^f - P_{\gB}^g \right) \right| \label{eqn. c1}\\
%	\leq& \int_{(\gX \times \gY)^2} \left| c_2 (Y^f, f^*(X)) - c_2(Y, f^*(X^g)) \right| d P^* (X, Y^f; X^g, Y) \label{eqn. c2} \\
%	=& \int_{{(\gX \times \gY)^2}} \left| c_2 (Y^f, f^*(X)) -  c_2 (Y^f, f^*(X^g)) {+} c_2 (Y^f, f^*(X^g)) - c_2(Y, f^*(X^g)) \right| d P^* (X, Y^f; X^g, Y) \nonumber\\
%	\leq& \int_{(\gX \times \gY)^2} \left| c_2 (Y^f, f^*(X)) {-} c_2 (Y^f, f^*(X^g)) \right| {+} \left| c_2 (Y^f, f^*(X^g)) {-} c_2(Y, f^*(X^g)) \right| d P^* (X, Y^f; X^g, Y) \nonumber\\
%	\leq& \int_{(\gX \times \gY)^2} \left[ L_{c_2} \left\| f^*(X) {-} f^*(X^g) \right\| {+}  c_2 (Y^f, Y) \right] d P^* (X, Y^f; X^g, Y) \label{eqn. c3}\\
%	\leq& \int_{(\gX \times \gY)^2} \left[ L_{1} \alpha c_1(X, X^g) {+} c_2 (Y^f, Y) \right] d P^* (X, Y^f; X^g, Y) {+} L_{1} M_1 \phi (\alpha)   \label{eqn. c4}\\
%	\leq& \int_{(\gX {\times} \gY)^2} \left[ c_1 (X^g, X) {+} c_2 (Y, Y^f) \right] d P^* (X, Y^f; X^g, Y) + L_{1} M_1 \phi(\alpha) \label{eqn. c5}\\
%	=& \gW (P_{\gA}^f, P_{\gB}^g) {+} L_{1} M_1 \phi(\alpha). \label{eqn. c6}
%	\end{align}
%	\end{small}
%    Line (\ref{eqn. c1}) follows by the definition of $ E_{\gA}^f (f^*) $ and $ E_{\gB}^g (f^*) $ and the definition of the expectation w.r.t. $ P_{\gA}^f $ and $ P_{\gB}^g $.
%    Line (\ref{eqn. c2}) holds by Lemma \ref{lemma:dual_KR} and we choose the optimal coupling $ P^* $, \textit{i.e.},
%    \begin{align*}
%	    P^* = \argmin\nolimits_{P \in \gP(P_{\gA}^f, P_{\gB}^g)} \E_{(X, Y'; X', Y) \sim P} [ c(X, Y'; X', Y) ].
%    \end{align*}
%	Line (\ref{eqn. c3}) holds by the $ L_{c_2} $-Lipschitz cost function $ c_2 $ w.r.t. the second argument, \textit{i.e.},
%	\begin{align*}
%	\left| c_2 (Y^f, f^*(X)) -  c_2 (Y^f, f^*(X^g)) \right| \leq L_{c_2} \left| f^*(X) - f^*(X^g) \right|,
%	\end{align*}
%	and the triangle inequality of the cost $ c_2 $, \textit{i.e.}, $ | c_2(Y^f, f^*(X^g)) - c_2(Y, f^*(X^g))| \leq c_2(Y^f, Y) $. 
%	Based on Definition \ref{def:probabilistic_Lipschitzness}, line (\ref{eqn. c4}) contains two cases: (1) $ f^* $ and $ \gP^* $ satisfies the  $ \phi $-probabilistic cross-domain Lipschitzness with probability $ 1 - \phi(\alpha) $; (2) the difference of $ f^* $ between any two instances is bounded by $ M_1 $, and we have the additional term $ L_{c_1} M_1 \phi (\alpha) $ that covers the regions where the $ \phi $-probabilistic cross-task Lipschitzness does not hold, \textit{i.e.}
%	\begin{align*}
%	& \int_{(\gX \times \gY)^2} L_{c_1} \left| f^*(X) - f^*(X^g) \right| d P^* (X, Y^f; X^g, Y) \\
%	\leq& \int_{(\gX \times \gY)^2} L_{c_1} \alpha c_2(X, X^g) d P^* (X, Y^f; X^g, Y) + L_{c_1} M_1 \phi (\alpha).
%	\end{align*}
%	Line (\ref{eqn. c5}) holds by the Lipschitz cost function $ c_1 $, and line (\ref{eqn. c6}) uses the definition of $ \gW (P_{\gA}^f, P_{\gB}^g) $.
%\end{proof}
%
%\begin{lemma}\label{Lemma:E_A_B}
%	Given Lipschitz cost function $ c_1 $ and $ c_2 $, and the input instances are bounded for $ f^* $ and $ g^* $, \textit{i.e.}, $ \|f^* (\bx_1) {-} f^* (\bx_2)\| \leq M_1 $ and $ \|g^* (\by_1) {-} g^* (\by_2)\| \leq M_2 $, if $   L_{c_1} \alpha {=} L_{c_2} \beta {=} 1 $, we have 
%	\begin{align*}
%	&E_{\gA}(f) \leq \gW_c (P_{\gA}^f, P_{\gB}^g) + L_{c_1} M_1 \phi (\alpha) + E_{\gA} (f^*) + E_{\gB}^g (f^*),\\
%	&E_{\gB}(g) \leq \gW_c (P_{\gA}^f, P_{\gB}^g) + L_{c_2} M_2 \phi (\beta)  + E_{\gB} (g^*) + E_{\gA}^f (g^*),
%	\end{align*}
%	with probability at least $ 1 - \delta $. 
%\end{lemma}
%\begin{proof}
%	Given $ E_{\gA}(f) = \E_{(X, Y) \sim P_{\gA}} \left[ c_2 (Y, f(X)) \right] $ and $ E_{\gB}(g) = \E_{(X, Y) \sim P_{\gB}} \left[ c_1 (X, g(Y)) \right] $, without loss of generality, we analyze the former as follows, and the latter is similar for the results.
%	\begin{align}
%	E_{\gA} (f)   
%	=& \E_{(X, Y) \sim P_{\gA}} \left[ c_2 (Y, f(X)) \right] \nonumber\\
%	=& \E_{(X, Y) \sim P_{\gA}} \left[ c_2 (Y, f^*(X)) + c_2 (f^*(X), f(X) ) \right] \label{l2eqn. 1}\\
%	=& \E_{(X, Y) \sim P_{\gA}} \left[ c_2 (f(X), f^*(X)) \right] + E_{\gA} (f^*)  \label{l2eqn. 2}\\
%	=& \E_{(X, Y) \sim P_{\gA}^f} \left[ c_2 (f(X), f^*(X) \right] + E_{\gA} (f^*) \label{l2eqn. 3} \\
%	=& E_{\gA}^f (f^*) + E_{\gA} (f^*)  \nonumber\\ 
%	=& E_{\gA}^f (f^*) - E_{\gB}^g (f^*) + E_{\gB}^g (f^*) + E_{\gA} (f^*)  \nonumber\\ 
%	\leq& \left| E_{\gA}^f (f^*) - E_{\gB}^g (f^*) \right| + E_{\gB}^g (f^*) + E_{\gA} (f^*) \label{l2eqn. 4} \\
%	\leq& \gW_c (P_{\gA}^f, P_{\gB}^g) + L_{1} M_1 \phi(\alpha) + E_{\gB}^g (f^*) + E_{\gA} (f^*).
%	\end{align}
%	Line (\ref{l2eqn. 1}) holds by an assumption that the loss function $ c_1 $ satisfies triangle inequality. 
%	Line (\ref{l2eqn. 2}) holds by a symmetric loss function $ c_1 $ and the definition of $ E_{\gA} (f^*) $, \textit{i.e.}, $ E_{\gA} (f^*) = \E_{(X, Y) \sim P_{\gA}} [c_2 (Y, f^*(X)] $.
%	Line (\ref{l2eqn. 3}) uses a fact that 
%	\begin{align*}
%	  \E_{(X, Y) \sim P_{\gA}} \left[ c_2 (f(X), f^*(X)) \right] 
%	= \E_{(X, f(X)) \sim P_{\gA}^f} \left[ c_2 (f(X), f^*(X)) \right] 
%	= E_{\gA}^f (f^*).
%	\end{align*}
%\end{proof}
%In order to prove Theorem \ref{theorem}, we introduce an important theorem that shows the concentration inequality for Wasserstein distance of the empirical measure and its true measure.
%\begin{thm} \emph{\textbf{(Empirical Concentration \cite{bolley-PTRF2007-quantitative}, Theorem 1.1)}}
%	\label{theorem: concentration_W}
%	Let $ \mu $ be a probability measure on $ \Omega $ 
%%	so that for some $ \rvw \in \Omega $, we have 
%%	\[\int e^{\tau d(\bw, \bw')^2} d \mu(\rvw) < +\infty,  \tau > 0 \]
%%	for any $ \rvw' \in \Omega $, 
%	and $ \hat{\mu} = \frac{1}{N} \sum_{i=1}^{N} \delta_{\rvw_i} $ be the associated empirical measure defined on a sample of independent variables $ \{\rvw_i\}_{i=1}^N $ drawn from $ \mu $. Then, for any $ d' > dim(\Omega) $ and $ C' < C $, there exists some constant $ N_0 $ depending on $ d' $ and some square exponential monments of $ \mu $ such that for any $ \epsilon > 0 $ and $ N \ge N_0 \max \{\epsilon^{-(d' + 2)}, 1\} $,
%	\begin{align*}
%	P\left[ \gW (\mu, \widehat{\mu}) > \epsilon \right] \leq e^{-\frac{C'}{2} N \epsilon^2},
%	\end{align*}
%	where $ C' $ can be calculated explicitly, and $ C $ is such that $ \mu $ verifies for any measure $ \nu $ the Talagrand (transportation) inequality $ T_1(C):  \gW(\mu, \nu) {\leq} {(\frac{2}{C} H(\nu|\mu))^\frac{1}{2}} $ with the relative entropy $ H $, and $ T_1(C) $ holds when for some $ \tau > 0 $ and $ \int e^{\tau d(\bw, \bw')^2} d \mu(\rvw) {<} {+}\infty, \forall\; \rvw' {\in} \Omega $.
%\end{thm}
%This theorem allows us to propose generalization bounds based on the Wasserstein distance.
%Now we can use this theorem and the previous Lemma to prove the following theorem.
%\begin{thm}\label{theorem}
%	Let $ P^* {=} \argmin_{P \in \gP(P_{\gA}^f, P_{\gB}^g)} \E_{(X, Y^f; X^g, Y) \sim P} [ c(X, Y^f; X^g, Y) ] $ with Lipschitz cost functions $ c_1 $ and $ c_2 $, and let functions $ f^* {\in} \gF $ and $ g^* {\in} \gG $ be probabilistic cross-domain Lipschitzness w.r.t. $ P^* $ that minimizes the joint error $ E(f^*, g^*) $, 
%	given $ M $ instances and $ N $ instances drawn form $ P_X $ and $ P_Y $, respectively, with $ L_{c_1} \alpha {=} L_{c_2} \beta {=} 1$, we have with probability at least $ 1 {-} \delta $:
%	\begin{align*}
%	E(f, g) \leq 2W_1 (\widehat{P}_{\gA}^f, \widehat{P}_{\gB}^g) + \sqrt{\frac{2}{C'} \log \left( \frac{2}{\delta} \right)} \left( \frac{2}{\sqrt{M}} + \frac{2}{\sqrt{N}} \right) + E(f^*, g^*) + \tilde{\phi} (\alpha, \beta), 
%	\end{align*}
%	where $ E(f^*, g^*) {=} E_{\gA} (f^*) {+} E_{\gB}^g (f^*) {+} E_{\gB} (g^*) {+} E_{\gA}^f (g^*) $, and $ \tilde{\phi} (\alpha, \beta) {=} L_{c_1} M_1 \phi (\alpha) {+} L_{c_2} M_2 \phi (\beta) $, where $ \| f^*(X_1) - f^*(X_2) \| \leq M_1, \forall X_1, X_2 \in \gX $ and $ \| g^*(Y_1) {-} g^*(Y_2) \| {\leq} M_2, \forall Y_1, Y_2 {\in} \gY $. Here, $ C' $ is some constant satisfying Theorem \ref{theorem: concentration_W}.
%\end{thm}
%\begin{proof}
%%	Let $ E(f^*, g^*) {=} E_{\gA} (f^*) {+} E_{\gB}^g (f^*) {+} E_{\gB} (g^*) {+} E_{\gA}^f (g^*) $, and $ \tilde{\phi} (\alpha, \beta) {=} L_{c_1} M_1 \phi (\alpha) {+} L_{c_2} M_2 \phi (\beta) $. 
%	Based on the definition of $ E(f, g) $, we have
%	\begin{align}
%	E(f, g) =& \E_{(X, Y) \sim P_{\gA}} \left[ c_2 (Y, f(X)) \right] + 
%	\E_{(X, Y) \sim P_{\gB}} \left[ c_1 (X, g(Y)) \right] \nonumber\\
%	\leq& 2 \gW (P_{\gA}^f, P_{\gB}^g) + E(f^*, g^*) + \tilde{\phi} (\alpha, \beta) \label{thm1:1}\\
%	\leq& 2 \gW (\widehat{P}_{\gA}^f, \widehat{P}_{\gB}^g) + \gW (\widehat{P}_{\gA}^f, P_{\gA}^f) \small{+} \gW (\widehat{P}_{\gB}^g, P_{\gB}^g) {+} E(f^*, g^*) {+} \tilde{\phi} (\alpha, \beta) \label{thm1:2}\\
%	\leq& 2 \gW (\widehat{P}_{\gA}^f, \widehat{P}_{\gB}^g) + \sqrt{\frac{2}{t'} \log \left( \frac{2}{\delta} \right)} \left( \frac{2}{\sqrt{M}} + \frac{2}{\sqrt{N}} \right) + E(f^*, g^*) + \tilde{\phi} (\alpha, \beta) \label{thm1:3}.
%	\end{align}
%	Line (\ref{thm1:1}) holds by the conclusion in Lemma \ref{Lemma:E_A_B}, and
%	line (\ref{thm1:2}) uses the triangle inequality for $ 1 $-Wasserstein distance.
%	In line (\ref{thm1:3}), we apply the union bound of $ \gW (\widehat{P}_{\gA}^f, P_{\gA}^f) $ and $ \gW (\widehat{P}_{\gB}^g, P_{\gB}^g) $ (with probability $ \frac{\delta}{2} $ for each) in Theorem \ref{theorem: concentration_W}.
%\end{proof}

\newpage
\section{Optimization Details}
In this section, we discuss some details of optimization for distribution divergence.
In the training, we use original GAN to measure the divergence $ d(P_X, Q_{X}) $, $ d(P_Y, Q_{Y}) $ and $ d(P_Z, Q_{Z}) $, respectively.

For $ d(P_X, Q_{X}) $, we optimize the following minimax problem:
\begin{align}
&\min_{F} \max_{D_x} \left[ \hat{\E}_{\bx \sim P_X} [\log D_x (\bx)] + \hat{\E}_{\tilde{\bx} \sim Q_X} [\log(1-D_x(\tilde{\bx}))] \right] \\
=&\min_{F} \max_{D_x}\left[ \hat{\E}_{\bx \sim P_X} [\log D_x (\bx)] + \lambda \hat{\E}_{{\bx} \sim P_X} [\log(1-D_x(G_1(E_2(G_2(E_1(\bx)))))))] + (1{-}\lambda) \hat{\E}_{{\by} \sim P_Y} (1{-}D_x(G_1(E_2(\by)))) \right],\nonumber
\end{align}
where $ D_x $ is a discriminator \wrt $ X $, and $ \lambda \in (0, 1) $.


For $ d(P_Y, Q_{Y}) $, we optimize the following minimax problem:
\begin{align}
&\min_{F} \max_{D_y} \left[ \hat{\E}_{\by \sim P_Y} [\log D_y (\by)] + \hat{\E}_{\tilde{\by} \sim Q_Y} [\log(1-D_y(\tilde{\by}))] \right] \\
=&\min_{F} \max_{D_y}\left[ \hat{\E}_{\by \sim P_Y} [\log D_y (\by)] + \lambda \hat{\E}_{{\by} \sim P_Y} [\log(1-D_y(G_2(E_1(G_1(E_2(\by)))))))] + (1{-}\lambda) \hat{\E}_{{\bx} \sim P_X} (1{-}D_y(G_2(E_1(\bx)))) \right],\nonumber
\end{align}
where $D_y$ is a discriminator \wrt $Y$, and $ \lambda \in (0, 1) $.


For $ d(P_Z, Q_{Z}) $, it contains $ d(P_Z, Q_{Z_1}) $ and $ d(P_Z, Q_{Z_2}) $ simultaneously, we optimize the following minimax problem:
\begin{align*}
	d(P_Z, Q_{Z_1}){=}\min_{E_1} \max_{D_z} \left[ \hat{\E}_{\bz \sim P_Z} [\log D_z (\bz)] + \hat{\E}_{{\bx} \sim P_X} [\log(1-D_z(E_1(\bx)))] \right],
\end{align*} 
where $D_z$ is a discriminator \wrt $Z$, and $ \rvz  $ is drawn from the prior distribution $ P_{Z} $.
Similarly, the another term $ d(P_Z, Q_{Z_2}) $ can be written as
\begin{align*}
d(P_Z, Q_{Z_2}){=}\min_{E_2} \max_{D_z} \left[ \hat{\E}_{\bz \sim P_Z} [\log D_z (\bz)] + \hat{\E}_{{\by} \sim P_Y} [\log(1-D_z(E_2(\by)))] \right].
\end{align*}
%Let $ {\gL_{z}}(E_1{,} E_2{,} G_1{,} G_1{,} D_{z}){=}{\gL_{z_1}}(E_1{,} E_2{,} G_2{,} D_{z}){+}{\gL_{z_2}}(E_1{,} E_2{,} G_1{,} D_{z}) $ be the final loss. %minimizing $ {\gL}_{z} $ is consistent with the shared-latent space assumption~\cite{liu2017unsupervised} that images of two different domains have the same latent representation distribution.
%Here, minimizing $ {\gL}_{z} $ is similar to~\cite{liu2017unsupervised} which uses VAE-like objective with the similar cycle-consistency constraint.
%Moreover, ~\cite{liu2017unsupervised} also optimize $ \gD_Z(P_Z, Q_{Z_1}) $ by VAE-like objective using the similar cycle constraint.

%\end{appendix}

